Stable and Efficient Shapley Value-Based Reward Reallocation for Multi-Agent Reinforcement Learning of Autonomous Vehicles

With the development of sensing and communication technologies in networked cyber-physical systems (CPSs), multi-agent reinforcement learning (MARL)-based methodologies are integrated into the control process of physical systems and demonstrate prominent performance in a wide array of CPS domains, such as connected autonomous vehicles (CAVs). However, it remains challenging to mathematically characterize the improvement of the performance of CAVs with communication and cooperation capability. When each individual autonomous vehicle is originally self-interest, we can not assume that all agents would cooperate naturally during the training process. In this work, we propose to reallocate the system's total reward efficiently to motivate stable cooperation among autonomous vehicles. We formally define and quantify how to reallocate the system's total reward to each agent under the proposed transferable utility game, such that communication-based cooperation among multi-agents increases the system's total reward. We prove that Shapley value-based reward reallocation of MARL locates in the core if the transferable utility game is a convex game. Hence, the cooperation is stable and efficient and the agents should stay in the coalition or the cooperating group. We then propose a cooperative policy learning algorithm with Shapley value reward reallocation. In experiments, compared with several literature algorithms, we show the improvement of the mean episode system reward of CAV systems using our proposed algorithm.

==> Todo.tex <==
1. The current algorithm definition needs to be improved:
(1). What is learned after this algorithm? Think about the objective: design a reward reallocation mechanism so the agents "learn" (before the training process, they do not naturally want to collaborate, though we assume collaborate is the "optimal" strategy, but the agents do not know) to corporate: this include two things--> the agent learn that form a grand coalition is the best; and under this grand coalition, they have a "close to NE" policy trained by the algorithm, a policy network.

(2). The current missing part of the algorithm: the agents learned policy \pi^i (s^C), this should be for different "C" set. But, do they compare the policies and value they compute at different "s^c", and see which one gives the largest value? How does the \pi (s^C) neural network looks like, what are the inputs and what are the outputs? The usual policy network deals with just "s" or "s_i", but "s^C" the dimension even changes according to the coalition definition "C" (for example, if joint state concatenated from all agents i in the coalition C), how does one policy neural network deals with it? The CAV experiments just directly goes to the grand coalition, without checking smaller coalition and compare the agents' policies under different coalitions. However, this is not what really defined in the algorithm or the paper. Needs to fix this inconsistency.

2. What if the convex game assumption fill, does the shapley value still provide something, i.e., some sort of meaningful reward allocation, like a reward that correctly measure the contribution of each agent, then agent can choose their best "team division" and policy according to the value? DO not get stuck by the "stable and efficient" reward allocation conclusion. It can be unstable, or maybe grand coalition is not the best coalition, the best way is the N agents are divided into several subsystems and each subsystem collaborate, etc. They are disjoint or disconnect subteams, etc. There can be more complicated scenarios.

3. Think about Cathy's question: she is really asking about (1)(2) and that needs to be clear to solve her intersection traffic control problem. Basically, the agents need to figure out and learn by themselves, who to collaborate with, if collaborate, what should be the policy. 

==> formulation_nucleolus.tex <==
\section{Problem Formulation}
\label{sec:formulation}
We first formulate the connected autonomous vehicles (CAVs) problem as a MARL problem. We consider $n$ agents (e.g., autonomous vehicles) in the agent set $\mathcal{N} = \{1, ..., n\}$. Each agent $i$ is associated with an action $a^i \in \mathcal{A}^i$ and a state $s^i \in \mathcal{S}^i$. The global joint state is $ s = (s^1, ..., s^n) \in \mathcal{S} \defeq \mathcal{S}^1 \times \cdots \times \mathcal{S}^n$. Similarly, the global joint action is $ a = (a^1, ..., a^n) \in \mathcal{A} \defeq \mathcal{A}^1 \times \cdots \times \mathcal{A}^n$. Each coalition has a stage-wise reward function $R(s, a, \mathcal{C})$, where we denote a subset of the vehicles $\mathcal{N}$ as a coalition $\mathcal{C}$. 
%The coalition $\mathcal{C}$'s stage-wise reward is $R(s, a, \mathcal{C})$. 
Specially, the $\mathcal{N}$ denotes the grand coalition in which all the $n$ agents cooperate together. Let $R(s,a, \mathcal{N})$ to represent the global stage-wise reward under the grand coalition. In this paper, we assume that all rewards are nonnegative. 

We consider each agent is associated with a localized policy $\pi^i(a^i| s^i)$ to choose a local action $a^i$ given its local state $s^i$. We use $\pi(a | s)= \prod_{i=1}^{n} \pi^i(a^i| s^i)$ to denote the joint policy, which is a product of the localized policies as each agent acts independently. The system's objective is to find a policy $\pi(a | s)$ to maximize the system's discounted total reward under the grand coalition, 
\begin{equation}
\label{equ:total_reward}
   \max_{\pi(a|s)} \Expect_{a_t \sim \pi(a|s)} \left[ \sum_{t=0}^\infty \gamma^t R_{t+1}(s_t, a_t, \mathcal{N}) | s_0 = s, a_0 = a \right],
\end{equation}
% \begin{equation}
%     \Expect_{a_t \sim \pi(a|s)} \left[ \sum_{t=0}^\infty \gamma^t R_{t+1}(s_t, a_t) | s_0 = s, a_0 = a \right],
% \end{equation}
where $\gamma$ is the discount factor. However, how to motivate agents to form a grand coalition has not been studied yet.

%This kind of stage-wise reward function can help improve the scalability in a large-scale system like connected autonomous vehicles~\cite{qu2020scalable}.

%Then we introduce the motivation to consider reward reallocation for cooperative policy learning of CAVs. 
The MARL problem is usually solved by the centralized training and decentralized execution paradigm that is first proposed in~\cite{lowe2017multi}. During training, there is a centralized critic $Q(s,a)$ that has access to the global state $s$ and global action $a$. This critic is used to train a localized actor for decentralized execution. However, having such a powerful centralized critic for autonomous vehicles is not easy, especially when each vehicle is self-interested and focuses to maximize its own reward (e.g., maximize its own driving speed or minimize its own travel time). Vehicles are not assumed to be fully cooperative.
Therefore, the goal of this paper is to design a better total reward reallocation mechanism, under which agents are willing to collaborate with each other by sharing their state and action information.
%we want to learn a cooperative localized policy $\pi^i(a^i|s^i)$ to encourage vehicles to form a large coalition $\mathcal{C}$ where they will share their states and actions with each other 
% for learning the approximated centralized $Q_{\pi^\mathcal{C}}(s^\mathcal{C}, a^\mathcal{C})$. Here, notation coalition $\mathcal{C}$ is a subset of the vehicles $\mathcal{N}$, $s^\mathcal{C}$ and $a^\mathcal{C}$ is the states and actions of the coalition that includes vehicle $i$, $\pi^\mathcal{C}(a^\mathcal{C} | s^\mathcal{C})= \prod_{i \in \mathcal{C}} \pi^i(a^i| s^i)$ is the joint policy of coalition $\mathcal{C}$. The coalition $\mathcal{C}$'s reward is $r^\mathcal{C} (s, a)= \sum_{i\in \mathcal{C}} r^i(s, a)$. For each vehicle $i \in \mathcal{C}$, they use $Q_{\pi^\mathcal{C}}(s^\mathcal{C}, a^\mathcal{C})$ to learn its policy $\pi^i(a^i| s^i)$. 
% During execution, they can also better utilize their coalition's states for decision making.

Simply using original action value function $Q(s,a)$ is not guaranteed to learn a policy where agents are willing to cooperate. In order to find a better total reward for policy learning, we formulate and analyze the game between CAVs using the cooperative game framework. We define a cooperative game $G = (\mathcal{N}, v)$, where $v$ is the characteristic function introduced in Section~\ref{sec:convex_game}. 
%Denote a subset of the vehicles $\mathcal{N}$ as a coalition $\mathcal{C}$. Let $s^\mathcal{C}$ and $a^\mathcal{C}$ to denote the states and actions of the coalition. 
Consider the entire MARL problem across all timesteps, the value of any coalition $\mathcal{C}$ is 
\begin{equation}
    v(\mathcal{C}|s, a) = \Expect_{\pi(a|s)} \left[ \sum_{t=0}^\infty \gamma^t R_{t+1}(s_t, a_t, \mathcal{C}) | s_0 = s, a_0 = a\right]. \nonumber
\end{equation}
% Moreover, we have the following proposition for this game:

% \begin{prop}\label{prop:value}
% In the cooperative game $(\mathcal{N}, v)$, for any coalition $\mathcal{C} \subseteq \mathcal{N}$, $s\in\mathcal{S}$, and $a\in\mathcal{A}$,
% \end{prop}
% %\begin{equation*}
% \songyang{\centerline{$v(\mathcal{C}|s, a) \geq \sum_{i\in\mathcal{C}} v(\{i\}|s, a) .$}}
% %\end{equation*}

% \begin{proof}
% For any coalition (subset of the agent set $\mathcal{N}$) $\mathcal{C} \subseteq \mathcal{N}$, 
% \begin{align}
%      &v(\mathcal{C}|s, a) = \Expect_{a_t \sim \pi(a|s)} \left[ \sum_{t=0}^\infty \gamma^t R_{t+1}(s_t, a_t, \mathcal{C}) | s_0 = s, a_0 = a\right] \nonumber \\
%     &= \sum_{i\in{\mathcal{C}}} \Expect_{a_t \sim \pi(a|s)} \left[ \sum_{t=0}^\infty \gamma^t r_{t+1}^{i} (s_t, a_t, \mathcal{C}) | s_0 = s, a_0 = a \right] \nonumber \\
%     & \geq \sum_{i\in{\mathcal{C}}} \Expect_{a_t \sim \pi(a|s)} \left[ \sum_{t=0}^\infty \gamma^t r_{t+1}^{i} (s_t, a_t, \{i\}) | s_0 = s, a_0 = a \right] \nonumber \\
%     % &= \sum_{i\in{\mathcal{C}}} \Expect_{a^k_i \sim \pi_i} \left[ \sum_{k=0}^\infty \gamma^k r_i^{k+1}| s_0 = s\right] \label{eq2}\\
%     & = \sum_{i\in{\mathcal{C}}} v(\{i\}|s, a).
%     %&= \sum_{i=1}^N v^i(\mathcal{N}|s). \label{eq3}
% \end{align}
% % The equality \eqref{eq1} is based on the Assumption \ref{assump:efficent_reward}.
% \end{proof}

% \textcolor{red}{There are two types of cooperation we can consider:
% \begin{enumerate}
%     \item At each timestep, $r_{t+1}^{i} (s_t, a_t, \mathcal{C}) \geq r_{t+1}^{i} (s_t, a_t, \{i\}) $. This requires the agent receives a larger reward at each timestep in coalition $\mathcal{C}$.
%     \item Only the total reward holds the inequality. (Hard to prove mathematically.) In this case, even though the agent may receive a smaller reward at a certain timestep, the expected total reward is larger. For example, when one vehicle yields to another vehicle that is leaving the highway, itself can achieve a larger average velocity as there is more space to accelerate.
% \end{enumerate}
% }

Specially, when $\mathcal{C} = \mathcal{N}$ we have 
\begin{equation}
    v(\mathcal{N}|s, a) = \Expect_{\pi(a|s)} \left[ \sum_{t=0}^\infty \gamma^t R_{t+1}(s_t, a_t, \mathcal{N}) | s_0 = s, a_0 = a\right]. \nonumber
\end{equation}
It shows the value of the grand coalition $\mathcal{N}$ is exactly the system's total reward. We want to find a stable and efficient total reward reallocation for this underlying game such that agents can learn a cooperative policy. In the following section, we show how to utilize Shapley value to solve this problem.

% \comment{Explain more here why we need to define $v(N)$; }
% We define the cooperative game as $(\mathcal{N}, v)$, where $v$ is the characteristic nonnegative value function in cooperative game theory defined as

% \begin{align}
%     & v(\mathcal{N}|s, a) \defeq \Expect_{a_t \sim \pi(a|s)} \left[ \sum_{t=0}^\infty \gamma^t R_{t+1}(s_t, a_t) | s_0 = s, a_0 = a\right] \nonumber \\
%     &= \sum_{i=1}^n \Expect_{a_t \sim \pi(a |s)} \left[ \sum_{t=0}^\infty \gamma^t r^i_{t+1}(s_t, a_t) | s_0 = s, a_0 = a \right] \nonumber \\
%     % &= \sum_{i=1}^n \Expect_{a^i_t \sim \pi^i(a^i|s^i)} \left[ \sum_{k=0}^\infty \gamma^t r^i_{t+1}(s^i_t, a^i_t) | s_0 = s, a_0 = a \right] \nonumber \\
%     &= \sum_{i=1}^n Q^i_{\pi}(s, a) \defeq \sum_{i=1}^n v(\{i\}|s, a).
% \end{align}

% Note that we define $v(\mathcal{N}|s, a)$ to be the action-value function in reinforcement learning. 

% By analysing this cooperative game, we show how to utilize Shapley value as a stable and efficient reward reallocation such that vehicles can learn a cooperative policy in the following section.

% \textcolor{red}{The only example for convex game I find in the literature is Airport game. If we define $R(s, a, \mathcal{C})= \min_{i\in \mathcal{C}} r^i(s, a, \mathcal{C})$ then it is a convex game with $v(\mathcal{C}\cup\mathcal{D}|s, a) + v(\mathcal{C}\cap\mathcal{D}|s, a) \ge v(\mathcal{C}|s, a) + v(\mathcal{D}|s, a)$.}

\section{Stable and Efficient Reward Reallocation}
\label{sec:reward_reallocation}

% Consider the cooperative game as $(\mathcal{N}, v)$ where $v$ is the characteristic value function, as follows: Given $s\in\mathcal{S}$, let $v(\mathcal{C}|s)= \Expect_{a^k_{\mathcal{C}} \sim \pi_{\mathcal{C}}} \left[ \sum_{k=0}^\infty \gamma^k r_{\mathcal{C}}^{k+1}| s_0 = s\right]$, for any $\mathcal{C}$ with $|\mathcal{C}|>1$, and $v_i(s)= v(\{i\}|s)= \Expect_{a^k_i\sim \pi_i} \left[ \sum_{k=0}^\infty \gamma^k r_i^{k+1}| s_0 = s\right]$. Then, the following proposition shows the relationship between the coalition value  $v(\mathcal{C}|s)$ and individual value $v_i(s)$.

% Let $v_i(\{a_{-i}^k\}_{k=0}^{\infty},s)= \Expect_{a^k_i \sim \pi_i} \left[ \sum_{k=0}^\infty \gamma^k r_i^{k+1}| s_0 = s, \{a_{-i}^k\}_{k=0}^{\infty}\right]$. Then

% Notice that $v(\mathcal{N}|s)$ is actually the state-value function in reinforcement learning and the proposition \ref{prop:value} implies that $v(\mathcal{N}|s) = \sum_{i=1}^N v_i(s)$. In the following, we present the convexity of the defined cooperative game.

We first define the Shapley value for the cooperative game $G(\mathcal{N}, v)$ defined in Section~\ref{sec:formulation} and show that the Shapley value satisfies the axioms for a fair reward reallocation. We then present the main results of this paper, Theorem~\ref{theorem:core}. According to Theorem~\ref{theorem:core}, the Shapley value is a stable and efficient reward reallocation if the game $G=(\mathcal{N}, v)$ is a convex game. Then we give an example of the convex game and design Algorithm~\ref{alg:actor-critic}. A stable solution means any agent cannot get more payoff if they leave the coalition. %It is a solution concept described by core in cooperative game theory~\cite{chalkiadakis2011computational}. 
For CAVs, a stable solution means that vehicles will stay within the coalition, communicate and cooperate with other coalition members to optimize the coalition-level objective. An efficient solution means the system's total reward is completely distributed to each agent for cooperative policy learning. 
%Hence, our reward reallocation mechanism provides a stable coalition structure that encourages agents to communicate and cooperate.

% \songyang{
% We consider the superadditive cover $G^* = (\mathcal{N}, v^*)$ of the game $G= (\mathcal{N}, v)$, where 
% \begin{equation}
%     v^*(\mathcal{C}) = \max_{\mathcal{CS} \in \mathcal{CS}_{\mathcal{C}}} \sum_{\mathcal{D} \in \mathcal{CS} } v(\mathcal{D}), 
% \end{equation}
% and $\mathcal{CS}_{\mathcal{C}}$ denotes the space of all coalition structures over $\mathcal{C}$. Intuitively, the value of a coalition $\mathcal{C}$ in $G^*$ is the maximum amount that the agents in $\mathcal{C}$ can make if they are free to choose their collaboration pattern.}

% \begin{lemma}
% If an outcome $(\mathcal{CS}, x)$ is in the core of the game $G^*= (\mathcal{N}, v^*)$, then $(\mathcal{CS}, x)$ is also in the core of the game $G= (\mathcal{N}, v)$.
% \end{lemma}
% \begin{proof}
% We first show that 
% Since the outcome $(\mathcal{CS}, x)$ is in the core of the game $G^*$, $x(\mathcal{C}) \geq v^*(\mathcal{C})$  for every $\mathcal{C} \subseteq \mathcal{N}$. Then we have $x(\mathcal{C}) \geq v^*(\mathcal{C}) = \max_{\mathcal{CS} \in \mathcal{CS}_{\mathcal{C}}} \sum_{\mathcal{D} \in \mathcal{CS} } v(\mathcal{D}) \geq v(\mathcal{C}).$
% Hence, $(\mathcal{CS}, x)$ is also in the core of the game $G= (\mathcal{N}, v)$.
% \end{proof}

We define the Shapley value of the game $G= (\mathcal{N}, v)$ as follows.
\begin{defi}[\textbf{Shapley Value}]
The Shapley value of the cooperative game $G= (\mathcal{N}, v)$ is defined to be
\begin{equation}
\label{equ:Shapley}
    \phi^i(s, a)\! \defeq \!\sum_{\mathcal{C}\subseteq \mathcal{N}\setminus\{i\}} \!\!\!\!\!\frac{|\mathcal{C}|!(n\!-\!|\mathcal{C}|\!-\!1)!}{n!} [v(\mathcal{C}\!\cup\! \{i\}|s, a) \!-\! v(\mathcal{C}|s,a)].
\end{equation}
\end{defi}

The Shapley value of the game $G= (\mathcal{N}, v)$ is extended for the multi-agent sequential decision problem. The intuition is that each agent's total reward is proportional to its contribution to the entire system. It is used to quantify the contribution of each agent for the communication-based cooperation in MARL. We show that the Shapley value satisfies the axioms for a fair reward reallocation as follows:

\begin{prop}
\label{prop:fairness}
The Shapley value of the cooperative game $(\mathcal{N},v)$ satisfies the following axiomatic characterization for a fair reward reallocation:
\begin{enumerate}
    \item Symmetric: if $v(\mathcal{C} \cup \{i\}|s, a) = v(\mathcal{C} \cup \{i\}| s, a)$ for any coalition $\mathcal{C} \subseteq \mathcal{N} \setminus\{i, j\}$, then $\phi^i(s, a) = \phi^j(s, a)$.
    \item Dummy player: if $v(\mathcal{C} \cup \{i\}|s, a) = v(\mathcal{C} | s, a)$ for any coalition $\mathcal{C} \subseteq \mathcal{N}$, then $\phi^i(s, a) = 0$. 
    \item Additivity: for any two $v^1$ and $v^2$, $\phi^i(s, a |v^1 + v^2) = \phi^i(s, a |v^1 ) + \phi^i(s, a | v^2)$ for each $i$, where $\phi^i(s, a |v^1 + v^2)$ is Shapley value of the game $(\mathcal{N}, v^1 + v^2)$ and $(v^1 + v^2)( \mathcal{C}|s, a) = v^1( \mathcal{C}|s, a) + v^2( \mathcal{C}|s, a)$.
\end{enumerate}
\end{prop}
\begin{proof}
Based on the definition of $\phi^i(s,a)$ in~\eqref{equ:Shapley}, we can derive the proposition above. 
\end{proof}

Besides fairness, we show that outcome $(\mathcal{N}, \phi)$ with Shapley value is an efficient outcome.
\begin{theorem} 
\label{theorem:core}
The outcome $(\mathcal{N}, \phi)$ with Shapley value is an efficient outcome of the cooperative game $G= (\mathcal{N}, v)$ and the Shapley value is an efficient reward reallocation.
\end{theorem}
\begin{proof}
Note that $v(\emptyset|s,a) \defeq 0$, then we have
\begin{align}
      \sum_{i \in \mathcal{N}} \phi^i(s, a) &= \sum_{i \in \mathcal{N}}  \sum_{\mathcal{C}\subseteq \mathcal{N}\setminus\{i\}} \!\!\!\!\!\frac{|\mathcal{C}|!(n\!-\!|\mathcal{C}|\!-\!1)!}{n!} [v(\mathcal{C}\!\cup\! \{i\}|s, a) \!\nonumber\\
      -\! v(\mathcal{C}|s,a)] &= n \frac{(n-1)!1!}{n!} v(\mathcal{N}|s,a) + n \frac{0!(n-1)!}{n!} v(\emptyset|s,a) \nonumber\\
    & + \sum_{\mathcal{C}\subset \mathcal{N}, \mathcal{C} \neq \emptyset, |\mathcal{C}|=p} ( p \frac{(p-1)!(n-p)!}{n!} -  \nonumber \\
    & (n-p) \frac{p!(n-p-1)!}{n!}) v(\mathcal{C}|s, a) \nonumber \\
    & = v(\mathcal{N}|s,a).
\end{align}
Note that the first equation is a telescoping sum where both $v(\mathcal{N}|s,a)$ and $v(\emptyset|s,a)$ appear once for each agent. The value of coalition $\mathcal{C}$ with $p$ agents appears $p$ times with positive sign, once for each agent in $\mathcal{C}$; it also appears $n-p$ times with negative sign, once for each agent not in $\mathcal{C}$.
\end{proof}

Moreover, If the cooperative game $G= (\mathcal{N}, v)$ is a convex game, we show that the Shapley value is a stable and efficient reward reallocation. A convex game is defined as follows:
\begin{defi}[\textbf{Convex Game}]
The cooperative game $(\mathcal{N},v)$ is a convex game if for any pair of coalitions $\mathcal{C},\mathcal{D}\subseteq \mathcal{N}$,
\begin{equation*}
    v(\mathcal{C}\cup\mathcal{D}|s, a) + v(\mathcal{C}\cap\mathcal{D}|s, a) \ge v(\mathcal{C}|s, a) + v(\mathcal{D}|s, a).
\end{equation*}
\end{defi}

Now we show the main result of our work. For a convex game, we have the following theorem that guarantees that the core is nonempty, and there exists a stable and efficient solution for reallocating $v(\mathcal{N}|s,a)$ to each individual agent to motivate cooperation. In the following Theorem~\ref{theorem:core}, we prove and analyze the properties of the Shapley value based reward reallocation mechanism.

\begin{theorem} 
\label{theorem:core}
If the cooperative game $G= (\mathcal{N}, v)$ is a convex game, the outcome $(\mathcal{N}, \phi)$ with Shapley value is in the core and the Shapley value is a stable reward reallocation.
\end{theorem}
\begin{proof}
Note that the Shapley value for the game $G = (\mathcal{N}, v)$ is 
\begin{equation}
    \phi^i(s, a)\! = \!\sum_{\mathcal{C}\subseteq \mathcal{N}\setminus\{i\}} \!\!\!\!\!\frac{|\mathcal{C}|!(n\!-\!|\mathcal{C}|\!-\!1)!}{n!} [v(\mathcal{C}\!\cup\! \{i\}|s, a) \!-\! v(\mathcal{C}|s,a)]. \nonumber
\end{equation}

We then show that Shapley value allocation lies in the core of game $(\mathcal{N},v)$. 

Let the payoff vector defined by the marginal contribution of each agent, i.e., $x^i = v(\mathcal{C}\cup \{i\}|s,a) - v(\mathcal{C}|s,a)$ for $i\in\mathcal{N}$. The goal is to prove that $x=(x^1,\ldots,x^n)$ is in the core. For any  coalition $\mathcal{C}=\{i^1,i^2,\ldots,i^k\} \subseteq \mathcal{N}= \{1, ..., n\}$, we can write $v(\mathcal{C})$ as follows by telescoping sum, 
\begin{align}
    & v(\mathcal{C}|s,a) = v(\{i^1\}|s,a)-v(\emptyset|s,a) + v(\{i^1,i^2\}|s,a) \nonumber \\
    &- v(\{i^1\}|s,a) +\cdots+v(\mathcal{C}|s,a) - v(\mathcal{C}\setminus\{i^k\}|s,a).
\end{align}

Without loss generality, we assume that $i^1<i^2<\cdots<i^k$. Then for each $j \in\{1,\ldots,k\}$, we let $\mathcal{D}=\{1, 2, \ldots, i^{j-1}\}$ and by the definition of convex games, 
\begin{align}
    &v(\{i^1,\ldots,i^{j-1},i^j\}|s,a) - v(\{i^1,\ldots,i^{j-1}\}|s,a) \nonumber\\
    \le\ & v(\{1,\ldots,i^{j-1},i^j\}|s,a ) - v(\{1,\ldots,i^{j-1}\}|s,a)\nonumber\\
    =\ &x^{i^j},\label{eq:thm1_shapley_core}
\end{align}
where the last equation is based on $x^{i^j} = v(\mathcal{D}\cup \{i^j\}|s,a) - v(\mathcal{D}|s,a)$. By summing up \eqref{eq:thm1_shapley_core} from $j=1$ to $k$, we have $v(\mathcal{C}|s,a)\le \sum_{j=1}^k x^{i^j} = x(\mathcal{C}|s,a)$. Therefore, $x$ is a stable solution in the core based on Definition~\ref{def:stable} and any coalition $\mathcal{C}$ will not have incentives to deviate from the grand coalition. Moreover, since Shapley value is a convex combination of our constructed $x$, and core is a convex set, Shapley value reallocation for the game is also stable and lies in the core. 

%Since the Shapley value is in the core, it is a stable and efficient reward reallocation.

% At last, we show that Shapley value is efficient, since for any coalition $\mathcal{C}$,
% \begin{equation}
%     x(\mathcal{C}|s,a)= \sum_{i \in \mathcal{C}} \phi^i(s,a) = \sum_{i \in \mathcal{C}} v(\{i\}|s, a) = v(\mathcal{C}|s,a).\nonumber
% \end{equation}
% Therefore, Shapley value is an efficient reward reallocation based on Definition~\ref{def:efficient}.
\end{proof}

Theorem~\ref{theorem:core} shows that for a convex game $G = (\mathcal{N}, v)$, Shapley value has good properties as it is stable and efficient. No agent wants to deviate from the grand coalition. Then, in this case, using the action value function $Q(s,a)$ for a policy learning may not be the best choice. We can reallocate the system's total reward to each agent using the Shapley value $\phi^i(s, a)$. It is fair, stable, and efficient total reward reallocation for a convex game. Now, we give an example for the convex game. 

\begin{prop}
\label{prop:convex_example}
When $R(s, a, \mathcal{C})= \sum_{i\in \mathcal{C}} R(s, a, \{i\})$ for any coalition $\mathcal{C} \subseteq \mathcal{N}$, the cooperative game $G =(\mathcal{N},v)$ is a convex game.
\end{prop}
\begin{proof}
For any coalition $\mathcal{C} \subseteq \mathcal{N}$, $s\in\mathcal{S}$, and $a\in\mathcal{A}$, we have
\begin{align}
\label{equ:characteristic}
     &v(\mathcal{C}|s, a) = \Expect_{a_t \sim \pi(a|s)} \left[ \sum_{t=0}^\infty \gamma^t R_{t+1}(s_t, a_t, \mathcal{C}) | s_0 = s, a_0 = a\right] \nonumber \\
    &= \sum_{i\in{\mathcal{C}}} \Expect_{a_t \sim \pi(a|s)} \left[ \sum_{t=0}^\infty \gamma^t R_{t+1}(s_t, a_t, \{i\}) | s_0 = s, a_0 = a \right] \nonumber \\
    & = \sum_{i\in{\mathcal{C}}} v(\{i\}|s, a).
    %&= \sum_{i=1}^N v^i(\mathcal{N}|s). \label{eq3}
\end{align}
Then we have for any pair of coalitions $\mathcal{C},\mathcal{D}\subseteq \mathcal{N}$,
\begin{align}
    & v(\mathcal{C}\cup\mathcal{D}|s, a) + v(\mathcal{C}\cap\mathcal{D}|s, a) \nonumber \\
    & = \sum_{i\in\mathcal{C}\cup\mathcal{D}} v(\{i\}|s, a) + \sum_{i\in\mathcal{C}\cap\mathcal{D}} v(\{i\}|s, a)\nonumber \\
    & = \left(\sum_{i\in\mathcal{C}} v(\{i\}|s, a) + \sum_{i\in\mathcal{D}\setminus \mathcal{C}} v(\{i\}|s, a) \right) + \sum_{i\in \mathcal{C}\cap\mathcal{D}} v(\{i\}|s, a)\nonumber \\
    % & = \sum_{i\in\mathcal{C}} v(\{i\}|s, a) + \left( \sum_{i\in\mathcal{D}\setminus \mathcal{C}} v(\{i\}|s, a) + \sum_{i\in \mathcal{C}\cap\mathcal{D}} v(\{i\}|s, a) \right)\nonumber \\
    & = \sum_{i\in\mathcal{C}} v(\{i\}|s, a) + \sum_{i\in\mathcal{D}} v(\{i\}|s, a) \nonumber \\
    &  \geq v(\mathcal{C}|s, a) + v(\mathcal{D}|s, a).
\end{align}
\end{proof}

Proposition~\ref{prop:convex_example} gives us one example of the convex game. There exits other kind of convex games. In Proposition~\ref{prop:convex_example}'s example, the Shapley value also has zero-complaint from each coalition. We check the complaint from each coalition based on the Definition~\ref{def:nucleolus} using Nucleolus. The Nucleolus is introduced based on deficit of $\mathcal{C}$ that measures $\mathcal{C}$'s incentive to deviate the current coalition~\cite{chalkiadakis2011computational}. It can also be regarded as the amount of "complaints" of $\mathcal{C}$ for a reward reallocation.

\begin{theorem}
\label{theorem:nucleolus}
When $R(s, a, \mathcal{C})= \sum_{i\in \mathcal{C}} R(s, a, \{i\})$ for any coalition $\mathcal{C} \subseteq \mathcal{N}$, the Shapley value and Nucleolus solution are the same and the value is $v(\mathcal{C}\cup \{i\}|s, a)$.
\end{theorem}
\begin{proof}
Since $v(\mathcal{C}|s, a) = \sum_{i\in{\mathcal{C}}} v(\{i\}|s, a)$ for any coalition $\mathcal{C} \subseteq \mathcal{N}$ (in Eq.~\eqref{equ:characteristic}), we have

\begin{align}
     \phi^i(s, a)\! =& \!\sum_{\mathcal{C}\subseteq \mathcal{N}\setminus\{i\}} \!\!\!\!\!\frac{|\mathcal{C}|!(n\!-\!|\mathcal{C}|\!-\!1)!}{n!} [v(\mathcal{C}\!\cup\! \{i\}|s, a) \!-\! v(\mathcal{C}|s,a)]\nonumber\\
     =& \sum_{p=1}^{n-1}\frac{p!(n-p-1)!}{n!} \!\!\!\sum_{\mathcal{C}\subseteq \mathcal{N}\setminus\{i\},|\mathcal{C}|=p} [v(\mathcal{C}\cup \{i\}|s, a) \nonumber\\
    & - v(\mathcal{C}|s, a)] + \frac{1}{n} v(\{i\}|s, a).  \label{thm1:eq1}
\end{align}

% \begin{align}
%     \phi^i(s) &= \sum_{\mathcal{C}\subseteq \mathcal{N}\setminus\{i\}} \frac{|\mathcal{C}|!(N-|\mathcal{C}|-1)!}{N!} [v(\mathcal{C}\cup \{i\}|s, a) - v(\mathcal{C}|s,a)]\nonumber\\
%     &= \sum_{\mathcal{C}\subseteq \mathcal{N}\setminus\{i\}} \frac{|\mathcal{C}|!(N-|\mathcal{C}|-1)!}{N!} \left[v( \{i\}|s,a)\right] \nonumber\\
%     &=v(\{i\}|s, a)= Q^i_{\pi}(s, a).
% \end{align}

Since $v(\mathcal{C}\cup \{i\}|s, a) - v(\mathcal{C}|s, a) = v(\{i\}|s, a) $ and the number of subsets $(\mathcal{C}\subseteq \mathcal{N}\setminus\{i\},|\mathcal{C}|=p)$ is $\binom{n-1}{p}$. Then, \eqref{thm1:eq1} can be rewritten as
\begin{align}
    &\phi^i(s, a) =  \sum_{p=1}^{n-1}\frac{p!(n-p-1)!}{n!} \frac{(n-1)!}{p!(n-p-1)!}v(\{i\}|s, a) \nonumber\\
    &+ \frac{1}{n} v(\{i\}|s, a) =v(\{i\}|s, a).
\end{align}

For any coalition $\mathcal{C}$, the deficit $d(\phi,\mathcal{C}|s, a) = v(\mathcal{C}|s, a)-\sum_{i\in\mathcal{C}} \phi^i(s, a) = 0$. Since Nucleolus is the unique way to divide the payoff of the grand coalition, then we can conclude that the Shapley value and Nucleolus solution are the same and the value is $v(\mathcal{C}\cup \{i\}|s, a)$.
\end{proof}

Theorem~\ref{theorem:nucleolus} shows the Nucleolus is the same with Shapley value when $R(s, a, \mathcal{C})= \sum_{i\in \mathcal{C}} R(s, a, \{i\})$. It also shows the reward reallocation using Shapley value also reduces the amount of complaint.

% \begin{theorem} 
% \label{theorem:optimal}
% Each agent's optimal policy is the same with the system's optimal policy, in other words,
% \begin{equation}
%     \pi_* = \argmax_{\pi}  \Expect_{a_t \sim \pi(a|s)} \left[ \sum_{t=0}^\infty \gamma^t R_{t+1}(s_t, a_t) | s_0 = s\right].
% \end{equation}
% \end{theorem}
% \begin{proof}
% Each agent $i$ is finding a policy to maximize its own localized expected reward, i.e., 
% \begin{equation}
%     \pi^i_* = \argmax_{\pi^i}  \Expect_{a_t \sim \pi(a|s)} \left[ \sum_{t=0}^\infty \gamma^t r^i_{t+1}(s^i_t, a^i_t) | s_0 = s\right].
% \end{equation}
% Therefore, we have
% \begin{align}
%     & \argmax_{\pi}  \Expect_{a_t \sim \pi(a|s)} \left[ \sum_{t=0}^\infty \gamma^t R_{t+1}(s_t, a_t) | s_0 = s\right] \nonumber \\
%     &= \argmax_{\pi} \sum_i  \Expect_{a_t \sim \pi(a|s)} \left[ \sum_{t=0}^\infty \gamma^t r^i_{t+1}(s^i_t, a^i_t) | s_0 = s\right] \nonumber \\
%     &= \sum_i \argmax_{\pi^i}  \Expect_{a_t \sim \pi(a|s)} \left[ \sum_{t=0}^\infty \gamma^t r^i_{t+1}(s^i_t, a^i_t) | s_0 = s\right]\nonumber \\
%     &= \pi_*.
% \end{align}
% \end{proof}


% \section{Second Trial}
% We can define Shapley Q-function to be 
% \begin{align}
%     Q^i_S(s,a) &= \sum_{\mathcal{C}\subseteq \mathcal{N}\setminus\{i\}} \frac{|\mathcal{C}|!(N-|\mathcal{C}|-1)!}{N!} \left[v(\mathcal{C}\cup \{i\}) - v(\mathcal{C})\right],
% \end{align}
% where
% \begin{align}
%     v(\mathcal{C}) &= Q^\mathcal{C}(s^\mathcal{C}, a^\mathcal{C}), \\
%     v(\mathcal{C}\cup \{i\}) &= Q^{\mathcal{C}\cup \{i\}}(s^{\mathcal{C}\cup \{i\}}, a^{\mathcal{C}\cup \{i\}}).
% \end{align}

% In implementation, we only plug in the information from coalition $\mathcal{C}$ to the ideal centralized critic $Q(s,a)$. Just use 0 to represent missing information.

% Problems:
% \begin{itemize}
%     \item It is not clear whether it is a convex game.
%     \item Cannot calculate Shapley value directly.
% \end{itemize}


==> introduction_short.tex <==
\section{introduction}
\label{sec:intro}
The rapid evolution of ubiquitous sensing, communication, and computation technologies has contributed to the revolution of cyber-physical systems (CPSs). Increasingly, Multi-agent reinforcement learning (MARL)-based methodologies demonstrate prominent decision-making performance in a wide array of CPS domains. Connected and autonomous vehicles (CAVs) is one such type of networked CPS and multi-agent system. The U.S. Department of Transportation (DOT) has estimated that DSRC vehicle-to-everything (V2V) communication can address up to 82\% of all crashes in the U.S. and potentially saving thousands of lives and billions of dollars~\cite{DSRC_standard}. Communication of basic safety messages (BSMs) benefits CAVs coordination and control approaches in scenarios such as cross intersections or lane-merging~\cite{Coordinate_CAV, CV_intersection, ort2018autonomous}, platoon and adaptive cruise control~\cite{cacc_platoon, savefuel_Karl, V2Vbenefit_platoon}. 

However, it remains challenging to formally characterize the improvement of learning-based decision-making for CAV systems with V2X connections, and to reallocate the system level benefit efficiently to motivate stable cooperation of individual autonomous vehicles. Existing learning-based planning or control approaches do not utilize communication or potential shared information for autonomous vehicles yet~\cite{waymo_rss19,RobustEndtoEnd_icra20,PredictPolicyLearn_LeCun,UCBFlow_iccps19}. How V2X communication benefits MARL or improves systems total reward and motivates cooperation has not been formally defined or quantified.

We propose to formally define and quantify the value of communication-based cooperation to MARL based on Shapley value~\cite{Shapley, ShapleyQ_aaai20}, and reallocate it as a reward to individual agent to motivate cooperation. It will build a research foundation to formally quantify the value of information sharing and motivate cooperation for the CAV research society, and the results can be leveraged to other networked CPS to better understand the benefits of cooperation. Our proposed approach includes the following three major novelties and contributions.
\begin{itemize}
    \item We formally define and quantify how to reallocate the total reward of the system to individual agent efficiently to motivate information sharing and stable cooperation among multi-agents.
    \item We define a convex game formulation to study the reward reallocation problem, and prove that Shapley value based reward reallocation (which equals to the $Q$ value of an individual agent) is located in the core of the convex game in Theorem~\ref{theorem:core}. Hence, each individual agent should cooperate to receive more reward. 
    \item We propose a cooperative policy learning with Shapley value reward allocation algorithm. In experiments, we show the improvement of system's total reward, velocity and comfort of CAV systems using the proposed algorithm.
\end{itemize}

\section{Related Work}
\label{sec: relate}
Cooperative games attract increasing research interests in MARL~\cite{zhang2019multi}. Existing works have been investigated to encourage every agent to work collaboratively by assigning rewards appropriately, such as a value decomposition network~\cite{sunehag2018value, rashid_nips20}, subtracting a counterfactual baseline~\cite{foerster2017counterfactual}, or an implicit method~\cite{NEURIPS2020_8977ecbb}. Multi-agent deep deterministic policy gradient (MADDPG) applies a centralized $Q$-function to address the problem caused by the non-stationary environment~\cite{lowe2017multi, iqbal2019actor}. Online learning with communicative actions~\cite{learnComm_nips16, learnComm_iclr19,communication_POMDP, Comm_MAplan, learnComm_MARL, attentionComm_nips18} has shown performance improvement over non-communicative agents. In all these works, agents are assumed to cooperate during training process, however, whether agents will cooperate or whether the cooperative coalition is \textbf{stable} has not been answered yet. 

Another related line of work is coalition formation games, where selfish and rational agents choose to participate in coalitions to maximize their own utility, through static and dynamic formation process.
For static formation, bargaining methods to achieve the agreement where no agents would deviate from the agreement \cite{okada96,madoc93}, Shapley value \cite{iman19}, core \cite{sandholm99,iman19} and kernel \cite{taase04} to acquire stable coalitions and fair payoff distribution methods are proposed. 
However, these methods do not apply to our setting because we consider a dynamic process.
Methods that be used for analyzing dynamic coalition formation includes Bayesian RL and MARL~\cite{chalkiadakis04,chalkiadakis07,Taywade21,liu2021a}. However, these works all use MARL as a tool to analyze the coalition formation game, while we consider the converse - we leverage analytical tools in cooperative game and coalition formation game for reward reallocation design in MARL.
%We consider a different problem in this work. We consider how to encourage cooperative policy learning in MARL using cooperative game as an analytical tool.
% \textcolor{blue}{However, for the dynamic process, both the time-varying coalition structure and the uncertainty of other agents' information and environmental changes increase the complexity of coalition formation games significantly.}

Shapley value~\cite{Shapley} is one classical method to divide the total payoff of all players in a cooperative game so that each player receives his or her fair payment. It uniquely provides an equitable assignment of values to agents and is also one metric to measure the importance and marginal contribution of each player to the system. 
%Recent literature on learning has developed a principled framework of ``data Shapley"~\cite{DataShapley_ml19} to address data valuation and ``feature Shapley"~\cite{ShapleyFeature_nips17} to measure the importance of features to supervised learning algorithms. 
Computing Shapley is still challenging and requires computing all the possible marginal contributions, which is exponentially large in the training process. Therefore, approximation methods to estimate the Shapley value of agents, data, and features have been designed and are presented in the game theory and machine learning literature~\cite{ShapleyQ_aaai20,computeShapley_13, DataShapley_ml19, ShapleyFeature_nips17}. However, in this work, we leverage the game property to derive the Shapley value analytically for a MARL problem and reduce the computational complexity significantly by avoiding traversing all possible marginal contributions.
% propose a reward reallocation method such that it is fair considering each agent's contribution to the entire system and also stable motivating agents to cooperate.

% \textcolor{blue}{The novelty of our approach...}

